Projected GANs Converge Faster

Generative Adversarial Networks (GANs) produce high-quality images but are challenging to train. They need careful regularization, vast amounts of compute, and expensive hyper-parameter sweeps. We make significant headway on these issues by projecting generated and real samples into a fixed, pretrained feature space. Motivated by the finding that the discriminator cannot fully exploit features from deeper layers of the pretrained model, we propose a more effective strategy that mixes features across channels and resolutions. Our Projected GAN improves image quality, sample efficiency, and convergence speed. It is further compatible with resolutions of up to one Megapixel and advances the state-of-the-art Fr\'echet Inception Distance (FID) on twenty-two benchmark datasets. Importantly, Projected GANs match the previously lowest FIDs up to 40 times faster, cutting the wall-clock time from 5 days to less than 3 hours given the same computational resources.

==> app_datasets.tex <==
\CHANGED{
\section{Additional Datasets}\label{sec:datasets}
- datasets 256x2
- we do not change the hyperparameters of projected gan, we simply train until convergence
- one each dataset, we report the lowest FID achieved in previous literature
- for both KITTI fisheye (a subset if KITTI-360) and ADE indoor, we train FastGAN as a baselines.

\begin{table}[]
\resizebox{\textwidth}{!}{%
\renewcommand*{\arraystretch}{1.2}
\begin{tabular}{@{}lccccc@{}}
\toprule
 & \textbf{LSUN cat} & \textbf{LSUN horse} & \textbf{ADE indoor} & \textbf{Flowers Full} & \textbf{KITTI fisheye} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Prev. SotA\\ (Approach)\end{tabular} & \begin{tabular}[c]{@{}c@{}}5.57\\ (ADM~\cite{Dhariwal2021ARXIV})\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.57 \\ (ADM~\cite{Dhariwal2021ARXIV})\end{tabular} & \begin{tabular}[c]{@{}c@{}}30.33 \\ (FastGAN~\cite{Liu2021ICLR})\end{tabular} & \begin{tabular}[c]{@{}c@{}}19.60 \\ (MSG-StyleGAN \cite{Karnewar2020CVPR})\end{tabular} & \begin{tabular}[c]{@{}c@{}}6.64 \\ (FastGAN~\cite{Liu2021ICLR})\end{tabular} \\
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
Projected GAN & \textbf{3.89} & \textbf{2.17} & \textbf{6.70} & \textbf{3.86} & \textbf{2.72} \\ \midrule
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \midrule
 & \textbf{STL-10} & \textbf{CUB200} & \textbf{Stanford Dogs} & \textbf{Stanford Cars} & \textbf{} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Prev. SotA\\ (Approach)\end{tabular} & \begin{tabular}[c]{@{}c@{}}25.32 \\ (TransGAN~\cite{Jiang2021ARXIV})\end{tabular} & \begin{tabular}[c]{@{}c@{}}11.25 \\ (FineGAN~\cite{Singh2019CVPR})\end{tabular} & \begin{tabular}[c]{@{}c@{}}25.66 \\ (FineGAN~\cite{Singh2019CVPR})\end{tabular} & \begin{tabular}[c]{@{}c@{}}16.03 \\ (FineGAN~\cite{Singh2019CVPR})\end{tabular} &  \\
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
Projected GAN & \textbf{13.68} & \textbf{2.79} & \textbf{11.75} & \textbf{2.09} & \textbf{} \\ \bottomrule
\end{tabular}
}
\vspace{1em}
\caption{\textbf{FID on Additional Datasets ($256^2$)}
Without any hyperparameter changes, Projected GAN outperforms the previous state-of-the art on all evaluated datasets.
}
\label{tab:metrics_smallhighres}
\end{table}
}

==> sec_checklist.tex <==
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section 4-5.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section 6.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section 6.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section 3.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{Code and models will be released upon publication.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section 3,4,5 and Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{For GAN experiments this is too computationally expensive.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{In this work, no new datasets were curated.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}
\end{enumerate}
